Political Bias and Factualness in News Sharing across more than 100,000 Online Communities

As civil discourse increasingly takes place online, misinformation and the polarization of news shared in online communities have become ever more relevant concerns with real world harms across our society. Studying online news sharing at scale is challenging due to the massive volume of content which is shared by millions of users across thousands of communities. Therefore, existing research has largely focused on specific communities or specific interventions, such as bans. However, understanding the prevalence and spread of misinformation and polarization more broadly, across thousands of online communities, is critical for the development of governance strategies, interventions, and community design. Here, we conduct the largest study of news sharing on reddit to date, analyzing more than 550 million links spanning 4 years. We use non-partisan news source ratings from Media Bias/Fact Check to annotate links to news sources with their political bias and factualness. We find that, compared to left-leaning communities, right-leaning communities have 105% more variance in the political bias of their news sources, and more links to relatively-more biased sources, on average. We observe that reddit users' voting and re-sharing behaviors generally decrease the visibility of extremely biased and low factual content, which receives 20% fewer upvotes and 30% fewer exposures from crossposts than more neutral or more factual content. This suggests that reddit is more resilient to low factual content than Twitter. We show that extremely biased and low factual content is very concentrated, with 99% of such content being shared in only 0.5% of communities, giving credence to the recent strategy of community-wide bans and quarantines.

==> 05_dataset_summary.tex <==


\section{Summary of Dataset}\label{sec:dataset_summary}
\galen{move and rename}
\galen{TODOS: merge descriptions of both community and user distributions, below, and shorten}
\galen{unless stated otherwise, we filter to subreddits that are active, \ie have at least one post per month.}
 

\xhdr{Diversity of Users} \galen{could roll this into the overview of users, above, then break `ideological consistency' into its own xhdr?}
How diverse are \reddit users, in terms of the political bias and factualness of their submissions to the communities they are members of? How ideologically consistent are users? In this analysis, we examine only users who submitted more than 10 links with a labeled bias/factualness value. We find that there is substantial variability across the mean bias and factualness of users' submitted links, but that both distributions of mean bias and mean factualness (\fig\ref{fig:distrib_of_means}) are far from uniform.

76\% of users have a mean bias between `center left' and `center', inclusive. Only 0.23\% of \reddit users (with more than 10 labeled links) have a mean bias more extreme than `left' or `right'. \galen{confusing wording, not sure how better to describe.} The distribution of mean factualness values is fairly similar to the mean bias distribution (\fig\ref{fig:distrib_of_means}). \tim{not sure what this means -- apples and oranges?} The vast majority (87\%) of users have a mean factualness between `mostly factual` and `high factual'. 

We measure a user's \textit{ideological consistency} \tim{this is a key construct and currently hidden in a summary section and subxhdr. Is there a good way to define key constructs and how they are measured first and do so clearly?} by computing the standard deviation of the political bias of their posts. We find that almost all users have some variance across their submissions, with only 1.3\% of users submitting only posts of a single bias category. The median user's standard deviation of political bias is 0.92. To give this some context, a user who mostly posts `center left' links, but posts one `center right' link for every 2.25 `center left' links would have a standard deviation of approximately 0.92. Alternately, a user who posts 100 `center left' links, 100 `center right' links, and 36 `center' links would have a standard deviation of .92. Alternately, a user who posts the same number of `left' links and `center' links would have a standard deviation of 1.0, a bit larger than our median user.  \galen{pick which examples to keep, if any.} \tim{it's great to put this in perspective. It may be easiest to just say: whatever the majority category of news for a user may be (eg., center left), on average they will post X\% in that majority category, Y\% in adjacent categories (e.g., left and center) and Y\% in the remaining categories (e.g., extreme left, center right, right, extreme right). (this might be simpler than the number games above.)}


\xhdr{Diversity of Communities}
How do communities vary in their political leaning? Their degree of factualness? How ideologically diverse are communities? As for users, we can operationalize communities' bias and factualness by computing the means thereof across all submissions to the community, and we can operationalize their (political) ideological diversity by computing the standard deviation of the the biases of all submissions to the community. \tim{Let's discuss listing and defining all key constructs in a prior section, possibly with mathematical notation.} Again, we limit our analysis to communities with at least 10 labeled links.

We find that the distribution of communities' mean bias and factualness values are very similar to those of users (\fig\ref{fig:distrib_of_means}), with 81\% of communities having a mean bias between `left center` and `center'. 87\% of communities have a mean factualness between `mostly factual' and `high factual', inclusive.\tim{I like this characterization much better than the 0.9x standard deviation since the latter depends on the -3...3 scale (which we have to define somewhere). Maybe we can define in that section what we mean by "adjacent" categories and then use this language throughout?}

The median community has a standard deviation of political bias of 0.95, very slightly \textit{greater} than that of the the median user. \tim{I wouldn't call attention to greater. It seems like a tiny difference.} Communities' content is of course submitted by community members who have their own ideological diversity; we explore the the ideological diversity of community members specifically below. \galen{segway.... diversity is similar to users, but given that community has multiple users, could come from blah.}
\tim{let me know when you reworked the section glue here.}



